Formal Verification of COO to CSR Sparse Matrix Conversion (Invited Paper)

We describe a machine-checked correctness proof of a C program that converts a coordinate-form (COO) sparse matrix to a compressed-sparse-row (CSR) matrix. The classic algorithm (sort the COO entries in lexicographic order by row,column; fill in the CSR arrays left to right) is concise but has rather intricate invariants. We illustrate a bottom-up methodology for deriving the invariants from the program.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{S.F.\ Siegel and G.\ Gopalakrishnan (Eds.):\\
International Workshop on Verification of\\
Scientific Software (VSS 2025)\\
EPTCS 432, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.432.3}{10.4204/EPTCS.432.3}}
\pdfoutput=1

